The Perceptual Observatory Characterizing Robustness and Grounding in MLLMs

Recent advances in multimodal large language models (MLLMs) have yielded increasingly powerful models, yet their perceptual capacities remain poorly characterized. In practice, most model families scale language component while reusing nearly identical vision encoders (e.g., Qwen2.5-VL 3B/7B/72B), which raises pivotal concerns about whether progress reflects genuine visual grounding or reliance on internet-scale textual world knowledge. Existing evaluation methods emphasize end-task accuracy, overlooking robustness, attribution fidelity, and reasoning under controlled perturbations. We present The Perceptual Observatory, a framework that characterizes MLLMs across verticals like: (i) simple vision tasks, such as face matching and text-in-vision comprehension capabilities; (ii) local-to-global understanding, encompassing image matching, grid pointing game, and attribute localization, which tests general visual grounding. Each vertical is instantiated with ground-truth datasets of faces and words, systematically perturbed through pixel-based augmentations and diffusion-based stylized illusions. The Perceptual Observatory moves beyond leaderboard accuracy to yield insights into how MLLMs preserve perceptual grounding and relational structure under perturbations, providing a principled foundation for analyzing strengths and weaknesses of current and future models.

==> sec/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> sec/prompts/gpg-query.tex <==
**INSTRUCTIONS**
You are given an image of size 1024x1024 that is composed of 4 sub-images arranged in a 2x2 grid as a collage.
Only one of these sub-images is the *source image* from which the support image was generated.

**TASK**
Identify and locate which grid cell contains the source image.
Coordinates mapping:
[0,0] = top-left
[0,1] = top-right
[1,0] = bottom-left
[1,1] = bottom-right

Return the result as valid JSON with detailed reasoning.

**JSON output format**
```json
{
  "reasoning": "Provide a structured explanation based on visual cues. Cite concrete visual evidence and justify your identification.",
  "final_answer": "[0,0]" or "[0,1]" or "[1,0]" or "[1,1]"
}
```



==> sec/prompts/gpg-support-celeb.tex <==
**CONTEXT**
You are given an image of size 1024x1024. This image is a visually altered version of some original image such that the source might contain a face of famous person that have been clearly visible, perturbed, stylized, or blended with the environment (background or object) as a visual illusion.
The information serves as the support context.


==> sec/prompts/gpg-support-word.tex <==
**CONTEXT**
You are given an image of size 1024x1024. This image is a visually altered version of some original image such that the source might contain a sequence of characters that are clearly written, perturbed, stylized, or blended with the environment (background or object) as a visual illusion.
The information serves as the support context.


==> sec/prompts/icl-analogy-partial-q3-query-celeb.tex <==
**INSTRUCTIONS**
You are given an image of size 1024x1024 that was generated from the above support image. A face is present in this image. The face might be clearly visible, perturbed, stylized, or blended with the environment (background or object) as a visual illusion.
The support context only consists of one key feature's bounding box.

**TASK**
Think and analyze the image carefully. Using the support context as a reference, detect the bounding boxes and provide detailed reasoning for each discernable facial attributes:
1. Left Eye
2. Right Eye
3. Nose
4. Mouth

Return the result as a valid JSON list. Your reasoning must explain how you identified the attribute, and only include the attribute that you can detect. If no attributes are confidently located, return empty list [].

**JSON output format**
```json
{
    "left_eye": {
        "reasoning": "Explain the visual evidence for this detection.",
        "x1": int,
        "y1": int,
        "x2": int,
        "y2": int
    },
    "right_eye": {
        "reasoning": "Explain the visual evidence for this detection.",
        "x1": int,
        "y1": int,
        "x2": int,
        "y2": int
    },
    "nose": {
        "reasoning": "Explain the visual evidence for this detection.",
        "x1": int,
        "y1": int,
        "x2": int,
        "y2": int
    },
    "mouth": {
        "reasoning": "Explain the visual evidence for this detection.",
        "x1": int,
        "y1": int,
        "x2": int,
        "y2": int
    }
}
```



==> sec/prompts/icl-analogy-partial-q3-query-word.tex <==
**INSTRUCTIONS**
You are given an image of size 1024x1024 that was generated from the above support image. The image contains a sequence of characters clearly written, distorted, stylized, or blended with the environment (background or object) as a visual illusion.
The support context only consists of top-left corner point of the bounding box.

**TASK**
Think and analyze the image carefully. Using the support context as a reference, detect the sequence of characters and provide a single bounding box that encloses all of its characters with detailed reasoning.

Return the result as a valid JSON list. If no sequence is confidently located, return empty list [].

**JSON output format**
```json
{
    "sequence": "The sequence of characters you read and detected",
    "reasoning": "Explain the visual evidence for this detection.",
    "x1": int,
    "y1": int,
    "x2": int,
    "y2": int
}
```



==> sec/prompts/icl-analogy-q3-query-celeb.tex <==
**INSTRUCTIONS**
You are given an image of size 1024x1024 that was generated from the above support image. A face is present in this image. The face might be clearly visible, perturbed, stylized, or blended with the environment (background or object) as a visual illusion.

**TASK**
Think and analyze the image carefully. Using the support context as a reference, detect the bounding boxes and provide detailed reasoning for each discernable facial attributes:
1. Left Eye
2. Right Eye
3. Nose
4. Mouth

Return the result as a valid JSON list. Your reasoning must explain how you identified the attribute, and only include the attribute that you can detect. If no attributes are confidently located, return empty list [].

**JSON output format**
```json
{
    "left_eye": {
        "reasoning": "Explain the visual evidence for this detection.",
        "x1": int,
        "y1": int,
        "x2": int,
        "y2": int
    },
    "right_eye": {
        "reasoning": "Explain the visual evidence for this detection.",
        "x1": int,
        "y1": int,
        "x2": int,
        "y2": int
    },
    "nose": {
        "reasoning": "Explain the visual evidence for this detection.",
        "x1": int,
        "y1": int,
        "x2": int,
        "y2": int
    },
    "mouth": {
        "reasoning": "Explain the visual evidence for this detection.",
        "x1": int,
        "y1": int,
        "x2": int,
        "y2": int
    }
}
```



==> sec/prompts/icl-analogy-q3-query-word.tex <==
**INSTRUCTIONS**
You are given an image of size 1024x1024 that was generated from the above support image. The image contains a sequence of characters clearly written, distorted, stylized, or blended with the environment (background or object) as a visual illusion.

**TASK**
Think and analyze the image carefully. Using the support context as a reference, detect the sequence of characters and provide a single bounding box that encloses all of its characters with detailed reasoning.

Return the result as a valid JSON list. If no sequence is confidently located, return empty list [].

**JSON output format**
```json
{
    "sequence": "The sequence of characters you read and detected",
    "reasoning": "Explain the visual evidence for this detection.",
    "x1": int,
    "y1": int,
    "x2": int,
    "y2": int
}
```



==> sec/prompts/icl-analogy-q3-support-celeb.tex <==
**CONTEXT**
You are given an image of size 1024x1024 of a famous person, "[CELEB_LABEL]". The following text provides context for the key features present in this image, listing each attribute with its precise bounding box coordinates. This information serves as a factual reference.

Attributes:
```json
[BBOX]
```


==> sec/prompts/icl-analogy-q3-support-word.tex <==
**CONTEXT**
You are given an image of size 1024x1024 of a case sensitive sequence of characters, "[WORD_LABEL]". The following text provides context for the sequence visible in this image, defining the characters and their precise bounding box. This information serves as a factual reference.

Attributes:
```json
[BBOX]
```


==> sec/prompts/image-matching-query.tex <==
**INSTRUCTIONS**
You are given 4 images each of size 1024x1024.

**TASK**
Compare the support image with 4 candidate images, and select a single candidate image that best matches the support image.

Return the result as valid JSON with detailed reasoning.

**JSON output format**
```json
{
  "reasoning": "Provide a structured explanation based on visual cues. Cite concrete visual evidence and justify your identification.",
  "final_answer": "A" or "B" or "C" or "D"
}
```

==> sec/prompts/image-matching-support-celeb.tex <==
**CONTEXT**
You are given an image of size 1024x1024 of a famous person. This information serves as a factual reference.
Additionally, you will further be given 4 images, only one of them is generated from this image, where a face might be clearly visible, perturbed, stylized, or blended with the environment (background or object) as a visual illusion.



==> sec/prompts/image-matching-support-word.tex <==
**CONTEXT**
You are given an image of size 1024x1024 of a case sensitive sequence of characters, "[WORD_LABEL]". This information serves as a factual reference.
Additionally, you will further be given 4 images, only one of them is generated from this image, where a sequence of characters are clearly written, perturbed, stylized, or blended with the environment (background or object) as a visual illusion.


